Discrete tensor product BGG sequences: splines and finite elements

In this paper, we provide a systematic discretization of the Bernstein-Gelfand-Gelfand (BGG) diagrams and complexes over cubical meshes of arbitrary dimension via the use of tensor-product structures of one-dimensional piecewise-polynomial spaces, such as spline and finite element spaces. We demonstrate the construction of the Hessian, the elasticity, and the divdiv complexes as examples for our construction.

==> FEM-H3-1d.tex <==
We now derive the finite element (FE) discretization for the one-dimensional BGG diagram~\eqref{diagram-1D} as well as the one-dimensional BGG complex~\eqref{BGG-complex1D}. First, we observe that the last element in the complex has regularity index $?-2$, meaning we loose two derivatives compared to the first element. As we cannot go below $L^2$, this implies that we must start with (at least) $H^2$ regularity on the left. 
Given $q=5$ (which ensures $r=2$ regularity), the proxy field FE-BGG diagram reads:
\begin{equation}
    \label{1D:high:BGG-diagram-FEM}
    \begin{tikzcd}
        0 \arrow{r} &\mathcal{S}^{5} (\mathcal{I}) \arrow{r}{\partial_x} &\mathcal{S}^{4} (\mathcal{I})\arrow{r}{} & 0\\
        0 \arrow{r} &\mathcal{S}^{4}(\mathcal{I})\arrow{r}{\partial_x} \arrow[ur, "Id"]&\mathcal{S}^{3}(\mathcal{I}) \arrow{r}{} & 0.
    \end{tikzcd}
\end{equation}
It is obtained starting from the following two proxy fields FE complexes
\begin{eqnarray}
    \label{1D:high:complex-FEM1} 
    \begin{tikzcd}
    0 \arrow{r}&\mathbb{R} \arrow{r}&\mathcal{S}^{5}(\mathcal{I}) \arrow{r}{\partial_x}& \mathcal{S}^{4}(\mathcal{I})\arrow{r}{}&0
    \end{tikzcd}
    \\
    \label{1D:high:complex-FEM2} 
    \begin{tikzcd}
    0 \arrow{r}&\mathbb{R} \arrow{r}&\mathcal{S}^{4}(\mathcal{I}) \arrow{r}{\partial_x}& \mathcal{S}^{3}(\mathcal{I})\arrow{r}{}&0
    \end{tikzcd}
\end{eqnarray} 
that have been presented in~\cite{Bonizzoni-Kanschat2022}. More in details, the spaces in the first FE complex are:
\begin{itemize}
    \item 
    $\mathcal{S}^{5}(\mathcal{I})$, equipped with the following set of node functionals
    \begin{gather*}
      \begin{aligned}
        \widetilde{\nodal^{0}_1}(u) &= u^\prime(0)& \qquad 
        \widetilde{\nodal^{0}_2}(u) &= u^\prime(1)\\
        \widetilde{\nodal^{0}_3}(u) &= u^{\prime\prime}(0)& \qquad 
        \widetilde{\nodal^{0}_4}(u) &= u^{\prime\prime}(1)\\
        \widetilde{\nodal^{0}_5}(u) &= u(1)-u(0) = \int_\interval u^\prime \, \dx& \qquad 
        \widetilde{\nodal^{0}_6}(u) &= u(1)+u(0)
      \end{aligned}
    \end{gather*}
    and the basis functions
    \begin{gather*}
      \begin{aligned}
        \widetilde{\phi^{0}_1}(x) &= -3x^5 + 8x^4 -6x^3+x& \qquad 
        \widetilde{\phi^{0}_2}(x) &= -3x^5+7x^4-4x^3\\
        \widetilde{\phi^{0}_3}(x) &= \frac{1}{2}x^5+\frac{3}{2}x^4-\frac{3}{2}x^3+\frac{1}{2}x^2& \qquad 
        \widetilde{\phi^{0}_4}(x) &= \frac{1}{2}x^5-x^4-\frac{1}{2}x^3\\
        \widetilde{\phi^{0}_5}(x) &= 6x^5-15x^4+10x^3-\frac{1}{2}& \qquad 
        \widetilde{\phi^{0}_6}(x) &= \frac{1}{2}
      \end{aligned}
    \end{gather*}
    
    \item 
    $\mathcal{S}^{4}(\mathcal{I})$, equipped with the following set of node functionals
    \begin{gather*}
      \begin{aligned}
        \widetilde{\nodal^{0}_1}(v) &= v(0)& \qquad 
        \widetilde{\nodal^{0}_2}(v) &= v(1)\\
        \widetilde{\nodal^{0}_3}(v) &= v^{\prime}(0)& \qquad 
        \widetilde{\nodal^{0}_4}(v) &= v^{\prime}(1)\\
        \widetilde{\nodal^{0}_5}(v) &= \int_\interval v \, \dx& \qquad 
        &
      \end{aligned}
    \end{gather*}
    and the basis functions $\widetilde{\phi^1_i}=d\widetilde{\phi^0_i}$ for all $i=1,\ldots,5$.
\end{itemize}
Concerning the second complex~\eqref{1D:high:complex-FEM2}, we have:
\begin{itemize}
    \item 
    $\mathcal{S}^{4}(\mathcal{I})$, equipped with the following set of node functionals
    \begin{gather*}
      \begin{aligned}
        \widehat{\nodal^{0}_1}(u) &= u^\prime(0)& \qquad 
        \widehat{\nodal^{0}_2}(u) &= u^\prime(1)\\
        \widehat{\nodal^{0}_3}(u) &= u(1)-u(0) = \int_\interval u^\prime \, \dx& \qquad 
        \widehat{\nodal^{0}_4}(u) &= \int_\interval x\, u^\prime(x)\, \dx\\
        \widehat{\nodal^{0}_5}(u) &= u(1)+u(0)& \qquad 
        &
      \end{aligned}
    \end{gather*}
    and the basis functions
    \begin{gather*}
      \begin{aligned}
        \widehat{\phi^{0}_1}(x) &= x^3-2x^2+x& \qquad 
        \widehat{\phi^{0}_2}(x) &= x^3-x^2\\
        \widehat{\phi^{0}_3}(x) &= -2x^3+3x^2-\frac{1}{2}& \qquad 
        \widehat{\phi^{0}_4}(x) &= \frac{1}{2}x^4-x^3+\frac{1}{2}x^2\\
        \widehat{\phi^{0}_5}(x) &= \frac{1}{2}& \qquad 
        &
      \end{aligned}
    \end{gather*}
    
    \item 
    $\mathcal{S}^{3}(\mathcal{I})$, equipped with the following set of node functionals
    \begin{gather*}
      \begin{aligned}
        \widehat{\nodal^{0}_1}(v) &= v(0)& \qquad 
        \widehat{\nodal^{0}_2}(v) &= v(1)\\
        \widehat{\nodal^{0}_3}(v) &= \int_\interval v(x)\, \dx& \qquad 
        \widehat{\nodal^{0}_4}(v) &= \int_\interval x\,v(x)\, \dx
      \end{aligned}
    \end{gather*}
    and the basis functions $\widehat{\phi^1_i}=d\widehat{\phi^0_i}$ for all $i=1,\ldots,4$.
\end{itemize}
It can be verified that the two FE complexes~\eqref{1D:high:interp-FEM1} and~\eqref{1D:high:complex-FEM2} are exact, so that Assumption~\ref{assump:1Dcomplex} is satisfied.

Given the above-mentioned node functionals, we can introduce the corresponding dual basis functions $\{\widetilde{\psi^0}_i\}_{i=1,\ldots,6}$ for $\mathcal S^5$, $\{\widetilde{\psi^1}_i\}_{i=1,\ldots,6}$ and $\{\widehat{\psi^0}_i\}_{i=1,\ldots,6}$ for $\mathcal S^4$, and $\{\widehat{\psi^1}_i\}_{i=1,\ldots,4}$ for $\mathcal S^3$, fulfilling
\begin{gather*}
    \begin{aligned}
      \widetilde{\nodal^0_j}(\widetilde{\psi^0_i})&=\delta_{i,j},&\qquad
      \widetilde{\nodal^1_j}(\widetilde{\psi^1_i})&=\delta_{i,j},&\qquad
      \widehat{\nodal^0_j}(\widehat{\psi^0_i})&=\delta_{i,j},&\qquad
      \widehat{\nodal^1_j}(\widehat{\psi^1_i})&=\delta_{i,j},
    \end{aligned}
\end{gather*}
for all admissible values of $i$ and $j$. The interpolation operators on the polynomial spaces of the first complex~\eqref{1D:high:complex-FEM1} are
\begin{gather}
    \label{1D:high:interp-FEM1}
    \widetilde{\interp^0}(u)\colon=\sum_{i=1}^6 \widetilde{\nodal^0_i}(u)\widetilde{\psi^0_i},\qquad
    \widetilde{\interp^1}(v)\colon=\sum_{i=1}^5 \widetilde{\nodal^1_i}(v)\widetilde{\psi^1_i},
\end{gather}
and those for the second complex are
\begin{gather}
    \label{1D:high:interp-FEM2}
    \widehat{\interp^0}(u)\colon=\sum_{i=1}^5 \widehat{\nodal^0_i}(u)\widehat{\psi^0_i},\qquad
    \widehat{\interp^1}(v)\colon=\sum_{i=1}^4 \widehat{\nodal^1_i}(v)\widehat{\psi^1_i}.
\end{gather}
The basis functions $\{\widetilde{\phi^\alpha}_i\}$ and $\{\widehat{\phi^\alpha}_i\}$, together with the node functionals $\{\widetilde{\nodal^\alpha}_i\}$ and $\{\widehat{\nodal^\alpha}_i\}$, with $\alpha=0,1$ and all admissible values of $i$, fulfill the assumption of the commuting Lemma 2 in~\cite{Bonizzoni-Kanschat2022}. Hence, the interpolation operators~\eqref{1D:high:interp-FEM1} and~\eqref{1D:high:interp-FEM2} commute with the  derivative, i.e., for all $u \in C^\infty(\interval)$, there holds
\begin{gather*}
    \partial_x \widetilde{\interp^0} u = \widetilde{\interp^1} \partial_x u, \qquad 
    \partial_x \widehat{\interp^0} u = \widehat{\interp^1} \partial_x u.
\end{gather*}
The node functionals $\{\widetilde{\nodal^\alpha}_i\}$ and $\{\widehat{\nodal^\alpha}_i\}$ are well-defined for smooth (namely, at least $C^q$) functions. However, as outlined in Remark 3 in~\cite{Bonizzoni-Kanschat2022}, weighted node functionals $\{\widetilde{\wnodal^\alpha}_i\}$ and $\{\widehat{\wnodal^\alpha}_i\}$ that are $L^2$-bounded can be introduced. This construction yields to  quasi-interpolation operators defined for all $u,v\in L^2(I)$ as:
\begin{gather}
    \label{1D:high:quasi-interp-FEM}
    \begin{aligned}
      \widetilde{\winterp^0}(u)\colon&=\sum_{i=1}^6 \widetilde{\wnodal^0_i}(u)\widetilde{\psi^0_i},\qquad
        \widetilde{\winterp^1}(v)\colon&=\sum_{i=1}^5 \widetilde{\wnodal^1_i}(v)\widetilde{\psi^1_i},\\
    \widehat{\winterp^0}(u)\colon&=\sum_{i=1}^5 \widehat{\wnodal^0_i}(u)\widehat{\psi^0_i},\qquad
        \widehat{\winterp^1}(v)\colon&=\sum_{i=1}^4 \widehat{\wnodal^1_i}(v)\widehat{\psi^1_i}.
    \end{aligned}
\end{gather}
It can be proved that the quasi-interpolation operators are $L^2$-stable and commute with the exterior derivative~\cite{bonizzoni2021h}. As a consequence, the set of quasi-interpolation operators defined over $L^2$-regular differential forms as
\begin{gather*}
    \begin{aligned}
        \pi^{0,0}(u)&\colon=\widetilde{\winterp^0}(u),\quad
        &\pi^{1,0}(u\, dx\otimes 1)&\colon=\widetilde{\winterp^1}(u)\, dx\otimes 1,\\
        \pi^{0,1}(u\, 1\otimes dx)&\colon=\widehat{\winterp^0}(u)\, 1\otimes dx,\quad
        &\pi^{1,1}(u\, dx\otimes dx)&\colon=\widehat{\winterp^1}(u)\, dx\otimes dx,
        \qquad \forall\, u\in L^2(\interval)
    \end{aligned}
\end{gather*}
satisfy Assumption~\ref{assump:interp}. 
\fbwarning{check the commutativity with $S^{0,1}$}
It remains us to check~\eqref{pis-spi}. 
About that, we note that the map $S^{0,1}$ in~\eqref{1D:high:BGG-diagram-FEM} represents the change of basis from $\{\widehat \phi^0_i\}_{i=1,\ldots,5}$ to $\{\widetilde \phi^1_i\}_{i=1,\ldots,5}$.


==> diagram-4.tex <==

%4-line diagram in 3D, iterative complexes. Conformal type complexes.

We consider the 4-row diagram in 3D:
 \begin{equation}\label{diagram-4rows-V}
\begin{tikzcd}
0 \arrow{r} &V^{0, 0} \arrow{r}{\grad} &V^{1, 0} \arrow{r}{\curl} & V^{2, 0} \arrow{r}{\div} & V^{3, 0} \arrow{r}{}& 0\\
0 \arrow{r}&
V^{0, 1}
\arrow{r}{\grad} \arrow[ur, "\mathrm{I}"]&
V^{1, 1}  \arrow{r}{\curl} \arrow[ur, "2\vskw"]&V^{2, 1}  \arrow{r}{\div} \arrow[ur, "\tr"]&V^{3, 1}  \arrow{r}{} & 0\\
0 \arrow{r}&
V^{0, 2}
\arrow{r}{\grad} \arrow[ur, "-\mathrm{mskw}"]&
V^{1, 2}  \arrow{r}{\curl} \arrow[ur, "\mathscr S"]&V^{2, 2}  \arrow{r}{\div} \arrow[ur, "2\vskw"]&V^{3, 2}  \arrow{r}{} & 0\\
0 \arrow{r} &V^{0, 3}\arrow{r}{\grad} \arrow[ur, "\iota"]&V^{1, 3} \arrow{r}{\curl} \arrow[ur, "-\mskw"]&V^{2, 3} \arrow{r}{\div}\arrow[ur, "I"] & V^{3, 3} \arrow{r}{} & 0.
 \end{tikzcd}
\end{equation}

According to the general framework, we have the following spaces. For the first row:
$$
V^{0, 0}=\mathcal S^{p_{1}, p_{2}, p_{3}}_{  \alpha_{1},  \alpha_{2},  \alpha_{3}},\quad V^{1, 0}=
\begin{pmatrix}
\mathcal S^{p_{1}-1, p_{2}, p_{3}}_{  \alpha_{1}-1,  \alpha_{2},  \alpha_{3}}\\
\mathcal S^{p_{1}, p_{2}-1, p_{3}}_{  \alpha_{1},  \alpha_{2}-1,  \alpha_{3}}\\
\mathcal S^{p_{1}, p_{2}, p_{3}-1}_{  \alpha_{1},  \alpha_{2},  \alpha_{3}-1}
\end{pmatrix},
$$
$$
V^{2, 0}=
\begin{pmatrix}
\mathcal S^{p_{1}, p_{2}-1, p_{3}-1}_{  \alpha_{1},  \alpha_{2}-1,  \alpha_{3}-1}\\
\mathcal S^{p_{1}-1, p_{2}, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2},  \alpha_{3}-1}\\
\mathcal S^{p_{1}-1, p_{2}-1, p_{3}}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}}
\end{pmatrix},\quad V^{3, 0}=\mathcal S^{p_{1}-1, p_{2}-1, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1}.
$$
For the second row, we employ the symmetry of the diagram to obtain
$$
V^{0, 1}= V^{1, 0} %=
%\begin{pmatrix}
%\mathcal S^{p_{1}-1, p_{2}, p_{3}}_{  \alpha_{1}-1,  \alpha_{2},  \alpha_{3}}\\
%\mathcal S^{p_{1}, p_{2}-1, p_{3}}_{  \alpha_{1},  \alpha_{2}-1,  \alpha_{3}}\\
%\mathcal S^{p_{1}, p_{2}, p_{3}-1}_{  \alpha_{1},  \alpha_{2},  \alpha_{3}-1}
%\end{pmatrix}
,\quad 
V^{1, 1}=
\begin{pmatrix}
\mathcal S^{p_{1}-2, p_{2}, p_{3}}_{  \alpha_{1}-2,  \alpha_{2},  \alpha_{3}} &\mathcal S^{p_{1}-1, p_{2}-1, p_{3}}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}}&\mathcal S^{p_{1}-1, p_{2}, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2},  \alpha_{3}-1} \\
\mathcal S^{p_{1}-1,p_{2}-1,p_{3}}_{  \alpha_{1}-1, \alpha_{2}-1, \alpha_{3}}&\mathcal S^{p_{1}, p_{2}-2, p_{3}}_{  \alpha_{1},  \alpha_{2}-2,  \alpha_{3}}&
\mathcal S^{p_{1}, p_{2}-1, p_{3}-1}_{  \alpha_{1},  \alpha_{2}-1,  \alpha_{3}-1}\\
\mathcal S^{p_{1}-1, p_{2}, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2},  \alpha_{3}-1} & \mathcal S^{p_{1}, p_{2}-1, p_{3}-1}_{  \alpha_{1},  \alpha_{2}-1,  \alpha_{3}-1}& \mathcal S^{p_{1}, p_{2}, p_{3}-2}_{  \alpha_{1},  \alpha_{2},  \alpha_{3}-2}
\end{pmatrix},
$$
$$
V^{2, 1}=
\begin{pmatrix}
\mathcal S^{p_{1}-1, p_{2}-1, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1} &\mathcal S^{p_{1}-2, p_{2}, p_{3}-1}_{  \alpha_{1}-2,  \alpha_{2},  \alpha_{3}-1}&\mathcal S^{p_{1}-2, p_{2}-1, p_{3}}_{  \alpha_{1}-2,  \alpha_{2}-1,  \alpha_{3}} \\
\mathcal S^{p_{1},p_{2}-2,p_{3}-1}_{  \alpha_{1}, \alpha_{2}-2, \alpha_{3}-1}&\mathcal S^{p_{1}-1, p_{2}-1, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1}&
\mathcal S^{p_{1}-1, p_{2}-2, p_{3}}_{  \alpha_{1}-1,  \alpha_{2}-2,  \alpha_{3}}\\
\mathcal S^{p_{1}, p_{2}-1, p_{3}-2}_{  \alpha_{1},  \alpha_{2}-1,  \alpha_{3}-2} & \mathcal S^{p_{1}-1, p_{2}, p_{3}-2}_{  \alpha_{1}-1,  \alpha_{2},  \alpha_{3}-2}& \mathcal S^{p_{1}-1, p_{2}-1, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1}
\end{pmatrix},\quad
V^{3, 1}=
\begin{pmatrix}
\mathcal S^{p_{1}-2, p_{2}-1, p_{3}-1}_{  \alpha_{1}-2,  \alpha_{2}-1,  \alpha_{3}-1}\\
\mathcal S^{p_{1}-1, p_{2}-2, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-2,  \alpha_{3}-1}\\
\mathcal S^{p_{1}-1, p_{2}-1, p_{3}-2}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-2}
\end{pmatrix}.
$$

For the third row: \gkerror{$V^{0,2}$ was wrong, now $V^{1,2}$ must be fixed. Is it the transpose of $V^{2,1}$?}
\dsnote{fixed $V^{1,2}$, $V^{2,2}$, $V^{3,2}$, and added the last row.}
$$
V^{0, 2}=V^{2, 0}
%\begin{pmatrix}
%\mathcal S^{p_{1}-1, p_{2}, p_{3}}_{  \alpha_{1}-1,  \alpha_{2},  \alpha_{3}}\\
%\mathcal S^{p_{1}, p_{2}-1, p_{3}}_{  \alpha_{1},  \alpha_{2}-1,  \alpha_{3}}\\
%\mathcal S^{p_{1}, p_{2}, p_{3}-1}_{  \alpha_{1},  \alpha_{2},  \alpha_{3}-1}
%\end{pmatrix}
,\quad 
V^{1, 2}=%V^{2, 1}
\begin{pmatrix}
\mathcal S^{p_{1}-1, p_{2}-1, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1} &\mathcal S^{p_{1}, p_{2}-2, p_{3}-1}_{  \alpha_{1},  \alpha_{2}-2,  \alpha_{3}-1} &\mathcal S^{p_{1}, p_{2}-1, p_{3}-2}_{  \alpha_{1},  \alpha_{2}-1,  \alpha_{3}-2} \\
\mathcal S^{p_{1}-2,p_{2},p_{3}-1}_{  \alpha_{1}-2, \alpha_{2}, \alpha_{3}-1}&\mathcal S^{p_{1}-1, p_{2}-1, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1}&\mathcal S^{p_{1}-1, p_{2}, p_{3}-2}_{  \alpha_{1}-1,  \alpha_{2},  \alpha_{3}-2}\\
\mathcal S^{p_{1}-2, p_{2}-1, p_{3}}_{  \alpha_{1}-2,  \alpha_{2}-1,  \alpha_{3}} & \mathcal S^{p_{1}-1, p_{2}-2, p_{3}}_{  \alpha_{1}-1,  \alpha_{2}-2,  \alpha_{3}}& \mathcal S^{p_{1}-1, p_{2}-1, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1}
\end{pmatrix},
$$

$$V^{2, 2}=
\begin{pmatrix}
\mathcal S^{p_{1}, p_{2}-2, p_{3}-2}_{  \alpha_{1},  \alpha_{2}-2,  \alpha_{3}-2} &\mathcal S^{p_{1}-1, p_{2}-1, p_{3}-2}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-2}&\mathcal S^{p_{1}-1, p_{2}-2, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-2,  \alpha_{3}-1} \\
\mathcal S^{p_{1}-1,p_{2}-1,p_{3}-2}_{  \alpha_{1}-1, \alpha_{2}-1, \alpha_{3}-2}&\mathcal S^{p_{1}-2, p_{2}, p_{3}-2}_{  \alpha_{1}-2,  \alpha_{2},  \alpha_{3}-2}&
\mathcal S^{p_{1}-2, p_{2}-1, p_{3}-1}_{  \alpha_{1}-2,  \alpha_{2}-1,  \alpha_{3}-1}\\
\mathcal S^{p_{1}-1, p_{2}-2, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-2,  \alpha_{3}-1} & \mathcal S^{p_{1}-2, p_{2}-1, p_{3}-1}_{  \alpha_{1}-2,  \alpha_{2}-1,  \alpha_{3}-1}& \mathcal S^{p_{1}-2, p_{2}-2, p_{3}}_{  \alpha_{1}-2,  \alpha_{2}-2,  \alpha_{3}}
\end{pmatrix}
%V^{2, 2}=
%\begin{pmatrix}
%\mathcal S^{p_{1}-1, p_{2}-1, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1} &\mathcal S^{p_{1}-2, p_{2}, p_{3}-1}_{  \alpha_{1}-2,  \alpha_{2},  \alpha_{3}-1}&\mathcal S^{p_{1}-2, p_{2}-1, p_{3}}_{  \alpha_{1}-2,  \alpha_{2}-1,  \alpha_{3}} \\
%\mathcal S^{p_{1},p_{2}-2,p_{3}-1}_{  \alpha_{1}, \alpha_{2}-2, \alpha_{3}-1}&\mathcal S^{p_{1}-1, p_{2}-1, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1}&
%\mathcal S^{p_{1}-1, p_{2}-2, p_{3}}_{  \alpha_{1}-1,  \alpha_{2}-2,  \alpha_{3}}\\
%\mathcal S^{p_{1}, p_{2}-1, p_{3}-2}_{  \alpha_{1},  \alpha_{2}-1,  \alpha_{3}-2} & \mathcal S^{p_{1}-1, p_{2}, p_{3}-2}_{  \alpha_{1}-1,  \alpha_{2},  \alpha_{3}-2}& \mathcal S^{p_{1}-1, p_{2}-1, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1}
%\end{pmatrix},
\quad
V^{3, 2}=
\begin{pmatrix}
\mathcal S^{p_{1}-1, p_{2}-2, p_{3}-2}_{  \alpha_{1}-1,  \alpha_{2}-2,  \alpha_{3}-2}\\
\mathcal S^{p_{1}-2, p_{2}-1, p_{3}-2}_{  \alpha_{1}-2,  \alpha_{2}-1,  \alpha_{3}-2}\\
\mathcal S^{p_{1}-2, p_{2}-2, p_{3}-1}_{  \alpha_{1}-2,  \alpha_{2}-2, \alpha_{3}-1}
\end{pmatrix}.
%V^{3, 2}=
%\begin{pmatrix}
%\mathcal S^{p_{1}-2, p_{2}-1, p_{3}-1}_{  \alpha_{1}-2,  \alpha_{2}-1,  \alpha_{3}-1}\\
%\mathcal S^{p_{1}-1, p_{2}-2, p_{3}-1}_{  \alpha_{1}-1,  \alpha_{2}-2,  \alpha_{3}-1}\\
%\mathcal S^{p_{1}-1, p_{2}-1, p_{3}-2}_{  \alpha_{1}-1,  \alpha_{2}-1, \alpha_{3}-2}
%\end{pmatrix}.
$$

$$ V^{0,3}=S^{p_1-1,p_2-1,p_3-1}_{  \alpha_{1}-1,  \alpha_{2}-1,  \alpha_{3}-1},\quad V^{1,3}= V^{3,1}, \quad V^{2, 3}=V^{3,2}, \quad
V^{3, 3}=\mathcal S^{p_{1}-2, p_{2}-2, p_{3}-2}_{  \alpha_{1}-2,  \alpha_{2}-2,  \alpha_{3}-2}.$$


\noindent For the spaces $V^{i,j}$ listed above, we may define the projection operators for each component $S_{\alpha_k,\alpha_l,\alpha_m}^{p_k,p_l,p_m}=S^{p_k}_{\alpha_k}\otimes S^{p_l}_{\alpha_l} \otimes S^{p_m}_{\alpha_m}$ as tensor products of $\tilde{\pi}_0^q$, $\tilde{\pi}_1^{q-1}$ and $\tilde{\pi}_2^{q-2}$. For example, $\tilde{\Pi}_{\cdot}:H^1(\mathcal{I}^3)\to S^{p_k,p_l,p_m}_{\alpha_k,\alpha_l,\alpha_m}$ is such that $\tilde{\Pi}_{\cdot}=\tilde{\pi}_{0}^{p_k} \otimes \tilde{\pi}_{1}^{p_l}\otimes \tilde{\pi}_{2}^{p_m}$. %Consider the projection operator for $V^{0,1}$. Using the operator $MAT: X^{3\times 3}\to  Y^{3\times 3}$ introduced in \cite{structure}, 
For $v\in V^{0,1}$, we define
\begin{align}
 \label{Tensorprodproj}
  \tilde{\Pi}v :&
  %= MAT(\tilde{\pi}_{1}^{p_1-1},\tilde{\pi}_{0}^{p_2},\cdots,\tilde{\pi}_{1}^{p_3-1})
    %(v_1,\cdots,v_9)
  %  \left(
  %  \begin{array}{c@{\otimes}c@{\otimes}c}
   % v_{11}&v_{12}&v_{13}\\ 
   % v_{21}&v_{22}&v_{23}\\
%    v_{31}&v_{32}&v_{33}
 %   \end{array}\right)
    = \left(
    \begin{array}{c@{\otimes}c@{\otimes}c}
   \tilde{\Pi}_1( v_{11}&v_{12}&v_{13})\\ 
    \tilde{\Pi}_2(v_{21}&v_{22}&v_{23})\\
   \tilde{\Pi}_3( v_{31}&v_{32}&v_{33})
    \end{array}\right) 
   \\ &:=\begin{pmatrix}
\tilde{\pi}_1^{p_1-1}(v_{11})\otimes \tilde{\pi}_{0}^{p_2}(v_{12})\otimes \tilde{\pi}_{0}^{p_3}(v_{13})\\
\tilde{\pi}_{0}^{p_1}(v_{21})\otimes \tilde{\pi}_1^{p_2-1}(v_{22}) \otimes \tilde{\pi}_{0}^{p_3}(v_{23})\\
\tilde{\pi}_{0}^{p_1}(v_{31})\otimes \tilde{\pi}_{0}^{p_2}(v_{32})\otimes \tilde{\pi}_1^{p_3-1}(v_{33}) \notag
\end{pmatrix} 
    \end{align}
%\noindent Then, assuming that each $v_i$ denotes %$S^{p_i}_{\alpha_i}$ for $i=1,2,3$, we may define the projection operators for $V^{0,1}$ as follows: 
%$$\tilde{\Pi}^0:= MAT(\tilde{\pi}_{0}^{p_1^1}, %\tilde{\pi}_{0}^{p_2^1}, %\tilde{\pi}_{0}^{p_3^1},\tilde{\pi}_{0}^{p_1^2}, %\tilde{\pi}_{0}^{p_2^2}, \tilde{\pi}_{0}^{p_3^2}, %\tilde{\pi}_{0}^{p_1^3}, \tilde{\pi}_{0}^{p_2^3}, %\tilde{\pi}_{0}^{p_3^3} ),$$ 
\noindent Similarly, we may define the operators for the other spaces $V^{i,j}$ given by a vector. For $V^{i,j}$ in matrix form such as $V^{1,1}$, we define the projection operator 
\begin{align*}
  \tilde{\Pi}v &:=[ \tilde{\Pi}_{\cdot 1} v_1,\tilde{\Pi}_{\cdot 2} v_2, \tilde{\Pi}_{\cdot 3} v_3] 
    \end{align*}
\noindent for $v=[v_1,v_2,v_3]\in V^{1,1}$. Note that $\tilde{\Pi}_{\cdot k}$ is a column vector defined similarly to $\tilde{\Pi}$ in Equation~\ref{Tensorprodproj}.


